Disjunctive Answer Set Solvers via Templates

Answer set programming is a declarative programming paradigm oriented towards difficult combinatorial search problems. A fundamental task in answer set programming is to compute stable models, i.e., solutions of logic programs. Answer set solvers are the programs that perform this task. The problem of deciding whether a disjunctive program has a stable model is $\Sigma^P_2$-complete. The high complexity of reasoning within disjunctive logic programming is responsible for few solvers capable of dealing with such programs, namely DLV, GnT, Cmodels, CLASP and WASP. In this paper we show that transition systems introduced by Nieuwenhuis, Oliveras, and Tinelli to model and analyze satisfiability solvers can be adapted for disjunctive answer set solvers. Transition systems give a unifying perspective and bring clarity in the description and comparison of solvers. They can be effectively used for analyzing, comparing and proving correctness of search algorithms as well as inspiring new ideas in the design of disjunctive answer set solvers. In this light, we introduce a general template, which accounts for major techniques implemented in disjunctive solvers. We then illustrate how this general template captures solvers DLV, GnT and Cmodels. We also show how this framework provides a convenient tool for designing new solving algorithms by means of combinations of techniques employed in different solvers.

==> section.5.extensions.tex <==
%\section{Perspectives}\label{sec:extensions}
\section{Extensions to the Framework}\label{sec:extensions}
In the following we present, in separate subsections, how three
enhancements implemented in disjunctive ASP solvers can be abstracted by
transition rules and added to the framework. %% These enhancements can be composed,
%% quite trivially by adding multiple subscripts, but the result would
%% be substantially more complicated than the template we defined.




\subsection{Early Minimality Tests}
{\gnt} implements an optimization technique which is not included in the techniques defined above: it performs an ``early'' minimality test in order to possibly backtrack earlier in the search if the current assignment does not lead to a solution. More precisely, given that these tests can be quite expensive, (as a further optimization) they are performed only when backtracking from a model candidate.

In order to model this technique, we define $\gntgraph{\aprogram}$ to be
$\simpletemplate{\smpropagators}{\smpropagators}{\thegengnt}{\thetestgnt}(\aprogram)$
in which the rule $\failright$ is replaced by the three right-rules
of Figure~\ref{fig:earlytests}.
Then, the graph $\gntgraph{\aprogram}$ is a more complete
representation of {\gnt} than the previous one we provided, as it includes early
minimality tests.

\begin{figure}
{\footnotesize
$$
\begin{array}{llll}
\earlytest
  & (\astringofliterals\decision{\aliteral}\astringofliterals',
     \anotherstringofliterals)_\rightstate
     & \transitionarrow
       (\astringofliterals\opposite{\aliteral},
        \emptyset)_\rightstate
        & \textrm{if}\left\{
          \begin{array}{l}
          \textrm{no other right-rule applies}
                       \textrm{ and}\\
          \anotherstringofliterals\textrm{ is consistent}
                       \textrm{ and}\\
          \decision{\aliteral}
                       \textrm{ is the rightmost decision literal of }
                       \astringofliterals\decision{\aliteral}\astringofliterals'
          \end{array}
          \right.\\ \\
\failright'
  & (\astringofliterals,
     \anotherstringofliterals)_\rightstate
     & \transitionarrow \terminalstate{\astringofliterals}
        & \textrm{if}\left\{
          \begin{array}{l}
          \anotherstringofliterals \textrm{ is inconsistent}
                       \textrm{ and}\\
          \anotherstringofliterals
                       \textrm{ contains no decision literal}
                       \textrm{ and}\\
          \astringofliterals
                       \textrm{ covers }\aprogram
          \end{array}
          \right.\\ \\
\failright''
  & (\astringofliterals,
     \anotherstringofliterals)_\rightstate
     & \transitionarrow
       (\astringofliterals,
        \emptyset)_\leftstate
        & \textrm{if}\left\{
          \begin{array}{l}
          \anotherstringofliterals \textrm{ is inconsistent}
                       \textrm{ and}\\
          \anotherstringofliterals
                       \textrm{ contains no decision literal}
                       \textrm{ and}\\
          \astringofliterals
                       \textrm{ does not cover }\aprogram
          \end{array}
          \right.
\end{array}
$$
}\normalsize
\label{fig:earlytests}
\caption{Early minimality test rules.}
\end{figure}

\yu{One of the issues that is there that EarlyTest is such that it creates a record on the left that does not cover atoms of Pi. The way we define witness function demands that it takes set of literals that covers Pi. There are rather many technical details discussed with respect to early minimality test in Gnt paper. I think we would have to be more detailed to include this discussion into the paper. As before I prefer to leave this section out.}

The $\earlytest$ rule prevents the rule $\backcross$ to be triggered when the
test on the right side fails. Instead, a new test, on a smaller instance, is
initiated.
Then the $\failright'$ rule is $\failright$ which avoids being triggered during
early minimality tests thanks to the third condition,
``$\astringofliterals$ covers $\aprogram$''.
Finally, during early minimality tests, if they succeed $\failright''$ can be
triggered.
Let us note that the rules $\failcross$ and $\backcross$ will only be triggered
when the early minimality test fails but there is no decision literal to further
do early minimality tests. Hence only $\failcross$ will ever be used,
$\backcross$ is subsumed by $\failright'$ and $\failright''$.

\begin{conjecture}~\label{thm:bbgraph}
For any $\aprogram$ the graph $\gntgraph{\aprogram}$
checks the stable models of $\aprogram$.
\end{conjecture}





\subsection{Separately Checking Non-Head-Cycle-Free Components}

In the {\dlv} implementation, the testing part is not always done ``one shot''
by creating a single CNF formula to be checked: however, if there are 
more than one non-head-cycle-free components, a CNF formula is created
for each component and tested. The hope is that the CNF formulas are
much easier to solve than the single formula, other than being smaller, and
also the process can terminate without checking all formulas.

In order to present this technique we need to introduce some other preliminaries.

A {\em cycle} of a program
$\aprogram$ is a list of atoms $\anatom_0,\dots,\anatom_\anotherindex$ such that w.r.t. any
$\anindex$, if $\anindex'=\anindex+1 (mod~\anotherindex +1)$, then there is a
rule $\ahead\aspimplication\abody$ of $\aprogram$ such that
$\anatom_{\anindex}\in\ahead$ and $\anatom_{\anindex'}\in\abody$.
A {\em loop} of the program $\aprogram$ is a set of atoms $\asetofatoms$ such
that there is an ordering of its elements that is a cycle of $\aprogram$.
We call $\loopset{\aprogram}$ the set of loops of $\aprogram$.
The {\em components} of a program $\aprogram$ are the maximal elements of
$\loopset{\aprogram}$ for $\subseteq$. The components of a program are
disjoint and their union is $\atoms{\aprogram}$.


A {\em head-cycle} in the program
$\aprogram$ is a cycle $\anatom_0,\dots,\anatom_\anotherindex$ in $\aprogram$
such that there are $\anindex$ and $\anindex'$ such that $\anatom_{\anindex}$
and $\anatom_{\anindex'}$ belong to the head of the same rule and
$\anatom_{\anindex}\neq\anatom_{\anindex'}$.
A component of a program $\aprogram$ is {\em head-cycle-free} if it
does not contain all the elements of any head-cycle of $\aprogram$;
we call $\hcfcomponents(\aprogram)$ the set of the head-cycle-free components of
$\aprogram$; and $\nonhcfcomponents(\aprogram)$ is the set of
the other components of $\aprogram$, that we call non-head-cycle-free
components. We assume that the set $\nonhcfcomponents(\aprogram)$ is ordered,
which allows us to call $\nonhcfcomponents(\aprogram,\anindex)$ the restriction
of $\aprogram$ to the atoms of the $\anindex^{\textrm{th}}$ non-head-cycle-free
component of a program.


We define $\thetestdlv_0$ to be $\thetestdlv$ modified so that,
when $\aprogram$ is head-cycle-free,
$\thetestdlv_0(\aprogram,\asetofliterals)=\emptyset$ if there is no
set unfounded on 
$\asetofliterals$ w.r.t. the program $\aprogram$, and
$\thetestdlv_0(\aprogram,\asetofliterals)=\{\aspimplication\}$ otherwise.
When $\aprogram$ is head-cycle-free,
checking whether there is a
set unfounded on 
$\asetofliterals$ w.r.t. the program $\aprogram$ can be done in polynomial time.
We now define $\dlvnewgraph{\aprogram}$ to be
$\simpletemplate{\smdisjpropagators}{\uppropagators}{\thegendlv}{\thetestdlv_0}(\aprogram)$
in which the states that were labelled by $\rightstate$ as
subscript are instead labelled by $\rightstate,\anindex$ where
$\anindex$ is an integer, and the rules $\crossrule$, $\failright$, $\propagateright$ and
$\backright$ are replaced by the rules of Figure~\ref{fig:separatecomponents}.
The other rules are unmodified, or handle the extra subscript in a trivial way.
Then the graph $\dlvnewgraph{\aprogram}$ is a better
representation of {\dlv} than the previous one we provided, as it includes
separate checking of non-head-cycle-free components.

\begin{figure}
{\footnotesize
$$
\begin{array}{llll}
\crossrule'
  & (\astringofliterals,
     \emptyset)_\leftstate
     & \transitionarrow
       (\astringofliterals,
       \emptyset)_{\rightstate,1}
       & \textrm{if}\left\{
          \begin{array}{l}
          \textrm{no left-rule applies}
          \end{array}
          \right.\\ \\
\failright'
  & (\astringofliterals,
     \anotherstringofliterals)_{\rightstate,\anindex}
     & \transitionarrow
       (\astringofliterals,
       \emptyset)_{\rightstate,\anindex+1}
        & \textrm{if}\left\{
          \begin{array}{l}
          \anotherstringofliterals \textrm{ is inconsistent}
                       \textrm{ and}\\
          \anotherstringofliterals
                       \textrm{ contains no decision literal}
                       \textrm{ and}\\
          \length{\nonhcfcomponents(\aprogram)}>\anindex
          \end{array}
          \right.\\ \\
\failright''
  & (\astringofliterals,
     \anotherstringofliterals)_{\rightstate,\anindex}
     & \transitionarrow \terminalstate{\astringofliterals}
        & \textrm{if}\left\{
          \begin{array}{l}
          \anotherstringofliterals \textrm{ is inconsistent}
                       \textrm{ and}\\
          \anotherstringofliterals
                       \textrm{ contains no decision literal}
                       \textrm{ and}\\
          \length{\nonhcfcomponents(\aprogram)}=\anindex
          \end{array}
          \right.\\ \\
% \backtrackright'
%   & (\astringofliterals,
%      \anotherstringofliterals\decision{\aliteral}\anotherstringofliterals')_{\rightstate,\anindex}
%      & \transitionarrow
%        (\astringofliterals,
%        \anotherstringofliterals\opposite{\aliteral})_{\rightstate,\anindex}
%         & \textrm{if}\left\{
%           \begin{array}{l}
%           \anotherstringofliterals\decision{\aliteral}\anotherstringofliterals'
%                         \textrm{ is inconsistent}
%                         \textrm{ and}\\
%           \anotherstringofliterals'\textrm{ contains no decision literal}
%           \end{array}
%           \right.\\ \\
\propagateright'
  & (\astringofliterals,
     \anotherstringofliterals)_{\rightstate,\anindex}
     & \transitionarrow
       (\astringofliterals,
       \anotherstringofliterals\aliteral)_{\rightstate,\anindex}
        & \textrm{if }\left\{
          \begin{array}{l}
          \aliteral\in\outprop{\asetofpropagators_\rightstate}
                              {\nonhcfcomponents(
                               \dependingprogram{\aprogram}{\astringofliterals},\anindex)}
                              {\anotherstringofliterals}
          \end{array}
          \right.\\
\end{array}
$$
}
\caption{Separate components rules.}
\label{fig:separatecomponents}
\end{figure}

The integer subscript of states labelled $\rightstate$ is representing which
non-head-cycle-free component is currently studied. Hence, the rule
$\propagateright'$ is reading only this component of
$\aprogram$ by using
$\dependingprogram{\nonhcfcomponents(\aprogram,\anindex)}{\astringofliterals}$,
and the rule $\crossrule'$ leads to the first component by using the integer $1$
as a subscript. The rule $\failright'$  is applied when one component is fully
explored so as to go to the next component, and the rule $\failright''$ is used
when all the components have been explored in order to return the final
result if no $\backtrackcross$ rule has been possible to apply in any of the
components.

\begin{conjecture}~\label{thm:clsepgraph}
For any $\aprogram$ the graph $\dlvnewgraph{\aprogram}$
checks the stable models of $\aprogram$.
\end{conjecture}










\subsection{Backjumping and Learning}
\label{subsec:bjandlearn}

In this section we show how to add backjumping and learning to the template.
Informally, {\em backjumping} does not always undo the previously made decision, as in
chronological backtracking used in classical {\dpll}, but is generally able to
backtrack further in the search tree by undoing several decisions at once. With
conflict-driven backjumping and {\em learning},
whenever backjumping is performed, a backjump clause, or here a backjump rule,
is learnt by adding it to a set of learnt clauses, or rules.
Learning clauses prevents a solver from reaching similar inconsistent
states in other parts of the search space. Backjumping and learning techniques are implemented by {\cmodels}, while {\dlv} implements only backjumping in~\cite{leo06}.


We now introduce some notations and concepts.

An {\em extended state} relative to sets $\asetofatoms$
and $\asetofatoms'$ is a pair
$(\astringofliterals\parallel\aprogram_\leftstate,\anotherstringofliterals\parallel\aprogram_\rightstate)_{\aside}$
or a distinguished state $\failstate$ or $\terminalstate{\astringofliterals}$,
where $\astringofliterals$
and~$\anotherstringofliterals$ are records relative to~$\asetofatoms$ and
$\asetofatoms'$ respectively, $\aprogram_\leftstate$ and $\aprogram_\rightstate$ are
sets of clauses $\aclause$ seen as program rules
$\aspimplication\opposite{\aclause}$
of which signature belongs to~$\asetofatoms$ and $\asetofatoms'$ respectively.
%% and $\aside\in\{\leftstate,\rightstate\}$ tells whether left or right rules
%% should be applied to this state.
The transitions of the template
$\simpletemplate{\asetofpropagators_\leftstate} {\asetofpropagators_\rightstate}
     {\themainprogram}{\thedependingprogram}$
we defined can be trivially extended to rules on extended
states, by converting any transition from
$(\asetofliterals_1,\asetofliterals_2)_{\aside}$
to
$(\asetofliterals_1',\asetofliterals_2')_{\aside'}$
(resp. to a terminal state)
into a transition from
$(\asetofliterals_1\parallel\aprogram_\leftstate,\asetofliterals_2\parallel\aprogram_\rightstate)_{\aside}$
to
$(\asetofliterals_1'\parallel\aprogram_\leftstate,\asetofliterals_2'\parallel\aprogram_\rightstate)_{\aside'}$
(resp. to the same terminal state).
Some extra care must be taken if $\asetofliterals_2$ (resp.
$\asetofliterals_2'$) is explicitly stated to be $\emptyset$: then the
corresponding extended state should be
$(\asetofliterals_1\parallel\aprogram,\emptyset\parallel\logicaltrue)$ (resp.
be $(\asetofliterals_1'\parallel\aprogram,\emptyset\parallel\logicaltrue)$).
We call this trivial extension of a transition rule its extended rule.
Finally, {\em initial state} is now referring to
$(\emptyset\parallel\logicaltrue,\emptyset\parallel\logicaltrue)_{\leftstate}$.

We can now add backjumping and learning rules in any of the graphs defined from the framework
$\simpletemplate{\asetofpropagators_\leftstate}
     {\asetofpropagators_\rightstate}
     {\themainprogram}{\thedependingprogram}$, by introducing the template $\learningtemplate
     {\asetofpropagators_\leftstate}
     {\asetofpropagators_\rightstate}
     {\themainprogram}{\thedependingprogram}(\aprogram)$.
For any two sets of
propagators $\asetofpropagators_\leftstate$ and $\asetofpropagators_\rightstate$, and any
generating and witness functions
$\themainprogram$ and $\thedependingprogram$,
the graph $\learningtemplate
     {\asetofpropagators_\leftstate}
     {\asetofpropagators_\rightstate}
     {\themainprogram}{\thedependingprogram}(\aprogram)$
is the graph in which the nodes are the extended states
     relative to $\atoms{\themainprogram(\aprogram)}$
     and $\atoms{\aprogram,\thedependingprogram}$, and the transitions rules are the
     extended rules of $\simpletemplate{\asetofpropagators_\leftstate}
     {\asetofpropagators_\rightstate}
     {\themainprogram}{\thedependingprogram}(\aprogram)$, with the two
     exceptions below:
\begin{enumerate}\itemsep0pt\parskip0pt\parsep0pt
  \item the $\learnleft$
     and $\learnright$ rules of Figure~\ref{fig:learnrules}, which are neither
     left-rules nor right-rules, are added; and
  \item
     $\propagateleft$, $\propagateright$, $\backtrackleft$, $\backtrackright$
     and $\backtrackcross$ rules are replaced by the $\propagateleft'$,
     $\propagateright'$, $\backjumpleft$, $\backjumpright$ and $\backjumpcross$
     rules of Figure~\ref{fig:learnrules}. $\backjumpleft$ and $\propagateleft'$
     are left-rules, while $\backjumpright$ and $\propagateright'$ are
     right-rules.
\end{enumerate}

The rules $\learnleft$ and $\learnright$ represent learning. At anytime a
consequence of the studied program can be learnt as a an additional rule in
$\aprogram_\leftstate$ or $\aprogram_\rightstate$, which will be used when
going through a $\propagateleft'$ or $\propagateright'$ rule as an extended
basis to apply the propagators of $\asetofpropagators_\genrighttest$ or
$\asetofpropagators_\genrighttest$ respectively. The $\learnleft$
and $\learnright$ rules are exclusively producing clauses $\aclause$ seen as rules
$\aspimplication\opposite{\aclause}$. The rules $\propagateleft'$ and
$\propagateright'$ are modified just for taking these clauses into account,
in the computation of
$\outprop{\asetofpropagators_\leftstate}
{\mainprogram{\aprogram}\setunion\aprogram_\leftstate}
{\astringofliterals}$
and
$\outprop{\asetofpropagators_\rightstate}
{\dependingprogram{\aprogram}{\astringofliterals}\setunion\aprogram_\rightstate}
{\anotherstringofliterals}$.
The rules $\backjumpleft$, $\backjumpright$ and $\backjumpcross$ replace
respectively $\backtrackleft$, $\backtrackright$ and $\backtrackcross$; they
allow, each in the same way, to backtrack further as per the backjumping idea.


Note that procedures built from 
the template will not necessarily use a polynomial
space since they store a possibly exponential amount of learnt rules.
Fixing this issue would involve the use and the adaptation of the techniques
used in~\cite{lier10}.


\begin{conjecture}~\label{STSL-correctness}
For any type $\atypeofmodel\in\{\classic,\supported\}$,
for any
$(\asetofpropagators_\genleftgen,\genleftgen)$
approximating-pair with respect to $\atypeofmodel$ and
$(\asetofpropagators_\genrighttest,\genrighttest)$
ensuring-pair with respect to $\atypeofmodel$,
for any $\aprogram$,
the graph
$\learningtemplate{\asetofpropagators_\genleftgen}{\asetofpropagators_\genrighttest}
                  {\genleftgen}{\genrighttest}(\aprogram)$
checks the stable models of $\aprogram$.
\end{conjecture}

\begin{figure}
\footnotesize{
$$
\begin{array}{llll}
\learnleft
  & (\astringofliterals\parallel\aprogram_\leftstate,
     \emptyset\parallel\emptyset)_\aside
     & \transitionarrow
       (\astringofliterals\parallel
        \aprogram_\leftstate\setunion\{\aspimplication\opposite{\aclause}\},
        \emptyset\parallel\emptyset)_\aside
        & \textrm{if}\left\{
          \begin{array}{l}
          \aclause \textrm{ is a logical consequence of }
             \mainprogram{\aprogram}\setunion\aprogram
                        \textrm{ and}\\
          \aclause \textrm{ does not occur in }
                        \aprogram
          \end{array}
          \right.\\ \\
\learnright
  & (\astringofliterals\parallel\aprogram_\leftstate,
     \anotherstringofliterals\parallel\aprogram_\rightstate)_\aside
     & \transitionarrow
       (\astringofliterals\parallel\aprogram_\leftstate,
        \anotherstringofliterals\parallel
        \aprogram_\rightstate\setunion\{\aspimplication\opposite{\aclause}\})_\aside
       & \textrm{if}\left\{
          \begin{array}{l}
          \aclause \textrm{ is a logical consequence of }
             \dependingprogram{\aprogram}{\astringofliterals}\setunion\aprogram
                        \textrm{ and}\\
          \aclause \textrm{ does not occur in }
                        \aprogram
          \end{array}
          \right.\\ \\

\propagateleft'
  & (\astringofliterals,
    \emptyset)_\leftstate
     & \transitionarrow
       (\astringofliterals\aliteral,
       \emptyset)_\leftstate
        & \textrm{if }\left\{
          \begin{array}{l}
          \aliteral\in\outprop{\asetofpropagators_\leftstate}
                              {\mainprogram{\aprogram}\setunion\aprogram_\leftstate}
                              {\astringofliterals}
          \end{array}
          \right.\\ \\

\backjumpleft
  & (\astringofliterals\decision{\aliteral}\astringofliterals'\parallel\aprogram_\leftstate,
     \emptyset\parallel\emptyset)_\leftstate
     & \transitionarrow
       (\astringofliterals\aliteral'\parallel\aprogram_\leftstate,
       \emptyset\parallel\emptyset)_\leftstate
        & \textrm{if}\left\{
          \begin{array}{l}
          \astringofliterals\decision{\aliteral}\astringofliterals'
                        \textrm{ is inconsistent}
                        \textrm{ and}\\
          \opposite{\astringofliterals}\logicalor\aliteral'
                        \textrm{ is a logical consequence of }
                        \mainprogram{\aprogram}\setunion\aprogram_\leftstate
          \end{array}
          \right.\\ \\

\propagateright'
  & (\astringofliterals,
     \anotherstringofliterals)_\rightstate
     & \transitionarrow
       (\astringofliterals,
       \anotherstringofliterals\aliteral)_\rightstate
        & \textrm{if }\left\{
          \begin{array}{l}
          \aliteral\in\outprop{\asetofpropagators_\rightstate}
                              {\dependingprogram{\aprogram}{\astringofliterals}\setunion\aprogram_\rightstate}
                              {\anotherstringofliterals}
          \end{array}
          \right.\\ \\

\backjumpright
  & (\astringofliterals\parallel\aprogram_\leftstate,
     \anotherstringofliterals\decision{\aliteral}\anotherstringofliterals'\parallel\aprogram_\rightstate)_\rightstate
     & \transitionarrow
       (\astringofliterals\parallel\aprogram_\leftstate,
       \anotherstringofliterals\aliteral'\parallel\aprogram_\rightstate)_\rightstate
        & \textrm{if}\left\{
          \begin{array}{l}
          \anotherstringofliterals\decision{\aliteral}\anotherstringofliterals'
                        \textrm{ is inconsistent}
                        \textrm{ and}\\
          \opposite{\anotherstringofliterals}\logicalor\aliteral'
                        \textrm{ is a logical consequence of }
          \dependingprogram{\aprogram}{\astringofliterals}\setunion\aprogram_\rightstate
          \end{array}
          \right.\\ \\
\backjumpcross
  & (\astringofliterals\decision{\aliteral}\astringofliterals'\parallel\aprogram_\leftstate,
     \anotherstringofliterals\parallel\aprogram_\rightstate)_\rightstate 
    & \transitionarrow
       (\astringofliterals \aliteral'\parallel\aprogram_\leftstate,
       \emptyset\parallel\emptyset)_\leftstate
        & \textrm{if}\left\{
          \begin{array}{l}
          \textrm{no right-rule applies}
                        \textrm{ and}\\
          \opposite{\astringofliterals}\logicalor\aliteral'
                        \textrm{ is a logical consequence of }
                        \mainprogram{\aprogram}\setunion\aprogram_\leftstate
          \end{array}
          \right.\\
\end{array}
$$
}\normalsize
\caption{Learning rules.}
\label{fig:learnrules}
\end{figure}



